Stellar abundance of binary stars: their role in determining the formation location of super-Earths and ice giants

Binary stars form from the same parent molecular cloud and thus have the same chemical composition. Forming planets take building material (solids) away from the surrounding protoplanetary disc. Assuming that the disc's accretion onto the star is the main process that clears the disc, the atmosphere of the star will show abundance reductions caused by the material accreted by the forming planet(s). If planets are only forming around one star of a binary system, the planet formation process can result in abundance differences in wide binary stars, if their natal protoplanetary discs do not interact during planet formation. Abundance differences in the atmospheres of wide binaries hosting giant planets have already been observed and linked to the formation location of giant planets. Here, we model how much building material is taken away for super-Earth planets that form inside/outside of the water ice line as well as ice giants forming inside/outside of the CO ice line. Our model predicts a significant abundance difference $\Delta$[X/H] in the stellar atmospheres of the planet-hosting binary component. Our model predicts that super-Earths that form inside the water ice line ($r<r_{\rm H_2O}$) will result in an $\Delta$[Fe/H]/$\Delta$[O/H] abundance difference in the their host star that is a factor of 2 larger than for super-Earths formed outside the water ice line ($r>r_{\rm H_2O}$) in the water rich parts of the disc. Additionally, our model shows that the $\Delta$[Fe/H]/$\Delta$[C/H] abundance difference in the host star is at least a factor of 3 larger for ice giants formed at $r<r_{\rm CO}$ compared to ice giants formed far out in the protoplanetary disc ($r>r_{\rm CO}$). Future observations of wide binary star systems hosting super-Earths and ice giants could therefore help to constrain the migration pathway of these planets and thus constrain planet formation theories.

==> ucs.tex <==
%%
%% This is file `ucs.sty',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% ucs.dtx  (with options: `ucs.sty')
%% 
%% Copyright 2001 Dominique Unruh  <unruh@ut.ee>
%% Copyright 2013 Wolfgang Jeltsch <wolfgang@cs.ioc.ee>
%% 
%% This program is provided under the terms of the LaTeX Project Public License with some
%% modifications. See the file LICENSE for information.
%% 
\catcode`\@11
\ifx\@gobble\undefined\def\@gobble#1{}\fi
\ifx\@gobbletwo\undefined\def\@gobbletwo#1#2{}\fi
\ifx\@gobblethree\undefined\def\@gobblethree#1#2#3{}\fi
\ifx\@gobblefour\undefined\def\@gobblefour#1#2#3#4{}\fi
\ifx\@firstofone\undefined\def\@firstofone#1{#1}\fi
\ifx\@tempcnta\undefined\csname newcount\endcsname\@tempcnta\fi
\ifx\@tempcntb\undefined\csname newcount\endcsname\@tempcntb\fi
\ifx\@testopt\undefined
  \def\@testopt#1#2{%
    \@ifnextchar[{#1}{#1[{#2}]}}\fi
\ifx\@protected@testopt\undefined\def\@protected@testopt{\expandafter\@testopt\@gobble}\fi
\let\@let@token\relax
\ifx\@ifnextchar\undefined
  \def\@ifnextchar#1#2#3{%
    \let\reserved@d=#1%
    \def\reserved@a{#2}%
    \def\reserved@b{#3}%
    \futurelet\@let@token\@ifnch}\fi
\ifx\@ifnch\undefined
  \def\@ifnch{%
    \ifx\@let@token\@sptoken
      \let\reserved@c\@xifnch
    \else
      \ifx\@let@token\reserved@d
        \let\reserved@c\reserved@a
      \else
        \let\reserved@c\reserved@b
      \fi
    \fi
    \reserved@c}\fi
\ifx\@inputcheck\undefined\newread\@inputcheck\fi
\ifx\IfFileExists\undefined
\long\def\IfFileExists#1#2#3{%
  \openin\@inputcheck#1 %SPACE
  \ifeof\@inputcheck\def\reserved@a{#3}%
  \else\closein\@inputcheck\def\reserved@a{#2}%
  \fi
  \reserved@a}%
\fi
\ifx\InputIfFileExists\undefined
\long\def\InputIfFileExists#1#2{%
  \IfFileExists{#1}{#2\input #1 }}
\fi
\ifx\protect\undefined\let\protect\relax\fi
\ifx\@typeset@protect\undefined\let\@typeset@protect\relax\fi
\ifx\IeC\undefined\def\IeC{\ifx\protect\@typeset@protect
  \expandafter\@firstofone\else\noexpand\IeC\fi}\fi
\def\unicode@knownoptions{}
\def\XDeclareUnicodeOption#1#2#3#4#5{%
  \expandafter\let\csname ifUnicodeOption#2\endcsname\iffalse
  \expandafter\def\csname UnicodeOption#2true%
    \expandafter\endcsname\expandafter{%
      \expandafter\let\csname ifUnicodeOption#2\endcsname\iftrue}%
  \expandafter\def\csname UnicodeOption#2false%
    \expandafter\endcsname\expandafter{%
      \expandafter\let\csname ifUnicodeOption#2\endcsname\iffalse}%
  \expandafter\def\csname @unicode@option@#2\endcsname{%
    #3\uni@activate@option{#2}{}{#4}{#5}}%
  \expandafter\def\csname @unicode@option@no#2\endcsname{%
    #3\uni@activate@option{#2}{no}{#4}{#5}}%
  \ifx~#1~\else\LinkUnicodeOptionToPkg{#2}{#1}\fi
  \let\uc@tempa\\\let\\\relax
  \edef\unicode@knownoptions{\\{#2}\unicode@knownoptions}%
  \let\\\uc@tempa
  }%
\let\uc@newcommand\def
\uc@newcommand\DeclareUnicodeOption{\@protected@testopt\DeclareUnicodeOption\DeclareUnicodeOption@{}}
\uc@newcommand\DeclareUnicodeOption@[#1]#2{%
  \XDeclareUnicodeOption{#1}{#2}{}{}{}}%
\uc@newcommand\uc@errormsg#1#2{%
  \ifx\PackageError\undefined
    {\newlinechar`\^^J\def\MessageBreak{^^J}%
      \errhelp{#2}\errmessage{Package ucs: #1}}%
  \else
    \PackageError{ucs}{#1}{#2}%
  \fi
}%
\uc@newcommand\uc@warnmsg#1{%
  \ifx\PackageWarning\undefined
    {\newlinechar`\^^J\def\MessageBreak{^^J}%
      \message{Package ucs: #1\MessageBreak}}%
  \else
    \PackageWarning{ucs}{#1}%
  \fi
}%
\def\uni@activate@option#1#2#3#4#5{%
  \ifx\uni@dataloaded\undefined
  \global\expandafter\def\csname @unicode@option@#1\endcsname##1{%
    \csname UnicodeOption#1true\endcsname
    \expandafter\def\csname uo-prio-#1\endcsname{##1}#3}%
  \global\expandafter\def\csname @unicode@option@no#1\endcsname##1%
    {\csname UnicodeOption#1false\endcsname#4}%
  \global\expandafter\let\csname uni@active@#1\endcsname1%
  \csname @unicode@option@#2#1\endcsname{#5}\else
  \uc@errormsg{Option #1 must be activated or deactivated %SPACE
    at least once in the preamble before using it in the document}{%
    For optimization causes I must know all %SPACE
    options before loading any unicode data.\MessageBreak
    Try e.g. #1 or no#1 as package option to ucs.}\fi}
\def\LinkUnicodeOptionToPkg#1#2{%
  \AtBeginDocument{\@ifpackageloaded{#2}{\SetUnicodeOption{#1}}{}}}%
\uc@newcommand\SetUnicodeOption{\@protected@testopt\SetUnicodeOption\SetUnicodeOption@{100}}
\uc@newcommand\SetUnicodeOption@[#1]#2{%
  \edef\uc@temp@a{@unicode@option@#2}%
  \expandafter\ifx\csname\uc@temp@a\endcsname\relax
    \PackageError{ucs}{Unknown unicode option #2}{}%
  \else
    \csname\uc@temp@a\endcsname{#1}%
  \fi}
\ifx\ProvidesPackage\undefined\else
\ProvidesPackage{ucs}[2013/05/11 v2.2 UCS: Unicode input support]%
\fi
\ifx\@@input\undefined\input uni-global.def \else\input{uni-global.def}\fi
\DeclareUnicodeOption{fasterrors}
\DeclareUnicodeOption{warnunknown}
\DeclareUnicodeOption{graphics}
\DeclareUnicodeOption{savemem}
\DeclareUnicodeOption{document}
\SetUnicodeOption[1000]{document}
\DeclareUnicodeOption{default}
\SetUnicodeOption[0]{default}
\XDeclareUnicodeOption{}{combine}{}{%
  \let\uc@cmb\empty}{%
  \ifx\unicodecombine\undefined\else\unicodecombine\fi
  \def\uc@cmb{\uc@warn@nocombine}}%
\ifx\AtBeginDocument\undefined\else
  \AtEndDocument{\unicodecombine}\fi
\SetUnicodeOption{nocombine}%
\def\uc@cmb{\uc@warn@nocombine}%
\ifx\DeclareOption\undefined\else
\DeclareOption{showmagickern}{\def\uc@magic@glue{6805678}}%
\DeclareOption{hyperref}{\AtEndOfPackage{\RequirePackage{ucshyper}}}%
\DeclareOption*{\SetUnicodeOption{\CurrentOption}}\ProcessOptions*
\fi
\ifx\AtBeginDocument\undefined
  \uc@warnmsg{Not loading ucsencs.def automatically.\MessageBreak
    Please load it after initializing fontencodings}%
\else
  \AtBeginDocument{\input{ucsencs.def}}\fi
\AtBeginDocument{\ifUnicodeOptiongraphics\RequirePackage{graphicx}\fi}%
\uc@newcommand\unicode@numtohex{\protect\unicode@numtohex@}%
\uc@newcommand\unicode@numtohex@#1#2#3{%
  {%\let\empty\relax\relax
   %\ifx\empty\relax\def\empty{}%
     \count255=#2\relax\gdef#1{}%
     \count252=#3%
     \loop
     \count253=\count252\advance\count253by\count255\relax
     \ifnum\count253>0%
     \ifnum\count252>0\advance\count252by-1\relax\fi
     \count254=\count255%
     \divide\count255by16%
     \multiply\count255by16%
     \advance\count254by-\count255%
     \xdef#1{\ifcase\count254 0\or1\or2\or3\or4\or5\or6\or7\or
       8\or9\or A\or B\or C\or D\or E\or F\fi#1}%
     \divide\count255by16\relax
     \repeat
   %\else
   %  \def#1{dec:#2}%
   %\fi
   }}
\let\uc@spc\space
\newcount\uc@secondtry
\uc@newcommand\unicode@invalid#1{%
  \unicode@combine%
  \ifUnicodeOptiongraphics{%
  \ifx\unicode@graphicsdir\undefined
    \def\unicode@graphicsdir{ucs-glyphs}\fi
  \ifx\unicode@graphicscmd\undefined
    \def\unicode@graphicscmd{ucs-getglyph \hex\space \dec\space \path\space}\fi
  \unicode@numtohex\hex{#1}4%
  \count255=#1\relax
  \divide\count255 by256\relax
  \unicode@numtohex\uc@temp@b{\count255}2%
  \edef\path{\unicode@graphicsdir/\uc@temp@b/U\hex.ps}%
  \edef\dec{\number#1}%
  \IfFileExists{\uc@temp@c}{}{%
    \typeout{Running: \unicode@graphicscmd}%
    \immediate\write18{\unicode@graphicscmd}%
    }%
 \IfFileExists{\path}{%
    \setbox255=\hbox{X}%
    \edef\uc@temp@b{\begingroup\noexpand\uni@resetcatcodes
      \noexpand\includegraphics[height=\the\ht255, trim=0 22.5 0 17.5]%
                      {\path}%
    \noexpand\ProvidesFile{U\hex.ps}%
        [Downloaded glyph for U+\hex]%
    \endgroup}%
  \typeout{\meaning\uc@temp@b}%
  \expandafter\unicodevirtual\expandafter{\uc@temp@b}%
  }{%
    \PackageWarning{ucs}{File \uc@temp@d\uc@temp@c.ps %SPACE
      not found.\MessageBreak
      Use\MessageBreak
      \space\space\space\space\unicode@graphicscmd\MessageBreak
      or start latex with option -shell-escape\MessageBreak
      if you have not already done so.}%
    \unicodevirtual{\unicode@invalidglyph{#1}}}}\else
    \unicodevirtual{\unicode@invalidglyph{#1}}\fi}
\uc@newcommand\unicode@invalidglyph#1{%
  {\unicode@numtohex\uc@temp@d{#1}4%
    \fontencoding{OT1}\texttt{[U+\uc@temp@d]}}}
\uc@newcommand\uni@char#1{%
  \ucs@protected@unichar\iftrue
    \expandafter\ifx\csname u-\number#1-h/o\endcsname\relax
  %    \end{macrocode}
  % If the character is not defined yet, load it.
  %    \begin{macrocode}
      \begingroup
        % In case \let is not executed, this (until ===) expands
        % to \let\relax\relax,
        % otherwise we have \let\uc@notloaderr\@gobble
        % Number of \empty's must equal number of args of \uc@char@notloaded
        \let\uc@notloaderr\@gobble\empty\@gobbletwo\relax\relax
        % ===
      \expandafter\endgroup
      % If \let not executed: Warning is emitted (see |\uc@notloaderr|)
      % otherwise: |\uc@char@notloaded| is called.
      \uc@notloaderr{\number#1}\uc@char@notloaded{#1}%
    \else
  %    \end{macrocode}
  % If the character is loaded, run |\uc@checkopts|
  % with the options of this character
  % as first arg and the code position as second; this will
  % display the character with
  % the correct option.
  %    \begin{macrocode}
     \expandafter\expandafter\expandafter\uc@checkopts
       \expandafter\expandafter\expandafter
       {\csname u-\number#1-h/o\endcsname}{#1}%
    \fi
  \else
    \noexpand\unichar{#1}%
  \fi
}
\begingroup
  \lccode`\A=`\{\lccode`\B=`\}\lccode`\C=`\\%
  \lccode`\P=`\P\lccode`\U=`\U%
  \lowercase{%
\endgroup
  \uc@newcommand\uc@notloaderr#1#2#3{%
    \ifx\@gobble#1\else[Please insert %SPACE
      CPrerenderUnicodeACunicharA#1BB into preamble]\fi}}
\uc@newcommand\uc@checkopts#1#2{%
  \expandafter\uc@checkopt@error\expandafter{\number#2}%
    {error}{error}{infinity}#1\@nil
}
\expandafter\uc@newcommand\csname uo-prio-infinity\endcsname{-2100000000}
%% === BEGIN AUTOGENERATED CODE
\uc@newcommand\uc@checkopt@stick#1#2#3#4#5{%
  \ifx\@nil#5%
\expandafter\ifx\csname u-#2-#1\endcsname\relax
  \uc@localdeferr{#1}{#2}%
\else
  \uc@output{\csname u-#2-#1\endcsname}{#1}%
\fi
    \expandafter\@gobblefour
  \else
    \iftrue\csname fi\endcsname
    \csname ifUnicodeOption#5\endcsname
      \ifnum\csname uo-prio-#2\endcsname>\csname uo-prio-#5\endcsname\uc@spc
        \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
        \uc@checkopt@stick
      \else
        \ifnum\csname uo-prio-#2\endcsname<\csname uo-prio-#5\endcsname\uc@spc
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \uc@checkopt@change
        \else
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \uc@checkopt@error
        \fi
      \fi
    \else
      \expandafter\expandafter\expandafter\uc@checkopt@stick
    \fi
  \fi
  {#1}{#2}{#5}{#2}%
}
\uc@newcommand\uc@checkopt@change#1#2#3#4#5{%
  \ifx\@nil#5%
\expandafter\ifx\csname u-#3-#1\endcsname\relax
  \uc@localdeferr{#1}{#3}%
\else
  \uc@output{\csname u-#3-#1\endcsname}{#1}%
\fi
    \expandafter\@gobblefour
  \else
    \iftrue\csname fi\endcsname
    \csname ifUnicodeOption#5\endcsname
      \ifnum\csname uo-prio-#3\endcsname>\csname uo-prio-#5\endcsname\uc@spc
        \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
        \uc@checkopt@stick
      \else
        \ifnum\csname uo-prio-#3\endcsname<\csname uo-prio-#5\endcsname\uc@spc
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \uc@checkopt@change
        \else
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \uc@checkopt@error
        \fi
      \fi
    \else
      \expandafter\expandafter\expandafter\uc@checkopt@stick
    \fi
  \fi
  {#1}{#3}{#5}{#3}%
}
\uc@newcommand\uc@checkopt@error#1#2#3#4#5{%
  \ifx\@nil#5%
\uc@errordrawopt{#1}{#2, #3}{#4}%
    \expandafter\@gobblefour
  \else
    \iftrue\csname fi\endcsname
    \csname ifUnicodeOption#5\endcsname
      \ifnum\csname uo-prio-#4\endcsname>\csname uo-prio-#5\endcsname\uc@spc
        \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
        \uc@checkopt@errorstick
      \else
        \ifnum\csname uo-prio-#4\endcsname<\csname uo-prio-#5\endcsname\uc@spc
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \uc@checkopt@change
        \else
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \uc@checkopt@error
        \fi
      \fi
    \else
      \expandafter\expandafter\expandafter\uc@checkopt@errorstick
    \fi
  \fi
  {#1}{#2, #3}{#5}{#4}%
}
\uc@newcommand\uc@checkopt@errorstick#1#2#3#4#5{%
  \ifx\@nil#5%
\uc@errordrawopt{#1}{#2}{#4}%
    \expandafter\@gobblefour
  \else
    \iftrue\csname fi\endcsname
    \csname ifUnicodeOption#5\endcsname
      \ifnum\csname uo-prio-#4\endcsname>\csname uo-prio-#5\endcsname\uc@spc
        \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
        \uc@checkopt@errorstick
      \else
        \ifnum\csname uo-prio-#4\endcsname<\csname uo-prio-#5\endcsname\uc@spc
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \uc@checkopt@change
        \else
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \uc@checkopt@error
        \fi
      \fi
    \else
      \expandafter\expandafter\expandafter\uc@checkopt@errorstick
    \fi
  \fi
  {#1}{#2}{#5}{#4}%
}
\let\unicode@empty\empty
\uc@newcommand\uc@errordrawopt#1#2#3{%
  \let\unicode@empty\relax\relax
  \ifx\unicode@empty\relax\let\unicode@empty\empty
    \unicode@numtohex\uc@temp@b{#1}4%
    \ifnum\csname uo-prio-#3\endcsname=-2100000000\relax
      \expandafter\ifx\csname
        missing-unicode-warned-\number#1\endcsname\relax
        \global\expandafter\let\csname
          missing-unicode-warned-\number#1\endcsname\@ne
        \unicode@error@unknown\@ne{Character \number#1\uc@spc
          \uc@spc= U+\uc@temp@b\uc@spc
          matches no activated options.\MessageBreak
          Type H to see available options}{#1}%
      \else
        \PackageWarning{ucs}{Character % SPACE
          \number#1 \uc@spc= 0x\uc@temp@b\uc@spc
          appeared again.}%
      \fi
    \else
      \@getcharinfo\uc@temp@c{#1}%
      \PackageWarning{ucs}{Character %SPACE
        \number#1 \uc@spc= 0x\uc@temp@b\uc@spc
        matches options\MessageBreak
        \uc@spc\uc@spc\uc@spc#2\MessageBreak
        with same priority \csname uo-prio-#3\endcsname. %SPACE
        Selecting option #3.\MessageBreak
        \uc@temp@c}%
      \uc@output{\csname u-#3-#1\endcsname}{#1}%
    \fi
  \else
    \noexpand\unichar{#1}%
  \fi
}
\uc@newcommand\uc@output#1#2{%
  \ifx\unicode@delay1\let\unicode@delay\relax\else
    \ifUnicodeOptioncombine
      \expandafter\uc@combine\expandafter{#1}{#2}%
    \else
      \uc@prechar@exec{#2}%
        \unicode@charfilter{#1{}}%
    \fi
    \ifx\uc@throw\undefined\else
      \def\uc@got{#2}\uc@throw\global\let\uc@throw\undefined\fi
  \fi
}%
\uc@newcommand\uc@prechar@exec#1{%
  \ifx\uc@prechar\undefined\else\uc@prechar{#1}\fi}
\uc@newcommand\uc@localdeferr#1#2{%
  \@getcharinfo\uc@temp@a{#1}%
  \PackageError{ucs}{Internal error in character \number#1, %SPACE
    option #2}{I probably got confused by intermixed local %SPACE
    and global definitions.\MessageBreak Try to load the needed %SPACE
    code page via \noexpand\PreloadUnicodePage
    before declaring anything by yourself.}{\uc@temp@a}%
  \unicode@invalid{#1}%
}%
\uc@newcommand\uc@warn@nocombine{%
  \PackageError{ucs}{Please activate option 'combine'}{Composed %SPACE
    characters can only be rendered correctly, when the option %SPACE
    'combine' is activated}}
\newtoks\uc@combtoks
\newtoks\uc@combtoksb
\newtoks\uc@temptokena
\uc@newcommand\unicode@combine{%
  \uc@check@magicglue%
  \ifx\uc@combining@prechar\undefined\global\let\uc@comb@code\undefined\fi
  \ifx\uc@comb@code\undefined\uc@temptokena{}\else
    \uc@temptokena\expandafter{\expandafter\uc@prechar@exec
      \expandafter{\uc@comb@code}}\fi%
  \global\let\uc@comb@code\undefined
  \global\expandafter\expandafter\expandafter\expandafter\expandafter
  \expandafter\expandafter\uc@combtoksb
  \expandafter\expandafter\expandafter
  \expandafter\expandafter\expandafter\expandafter{%
    \expandafter\expandafter\expandafter\the
    \expandafter\expandafter\expandafter\uc@combtoksb
    \expandafter\the\expandafter\uc@temptokena\the\uc@combtoks}%
  \global\uc@combtoks{}}
\def\uc@magic@glue{5381}
\uc@newcommand\uc@check@magicglue{%
  \ifnum\lastskip=\uc@magic@glue\unskip\else
    \begingroup
      \edef\uc@temp@a{\the\uc@combtoks}%
      \ifx\uc@temp@a\empty\else
      \PackageWarning{ucs}{Magic kern expected. Probably some %SPACE
        non-unicode characters mixed in while option combine was %SPACE
        in effect.}\fi\endgroup
  \fi}
\uc@newcommand\unicodevirtual#1{%
  \def\uc@temp@a##1{#1}\uc@output{\csname uc@temp@a\endcsname}{"FFFF}}
\uc@newcommand\unicodecombine{%
  \ifx\protect\@typeset@protect
    \unicode@combine%
    %\typeout{WRITING: \the\uc@combtoksb}%
    \the\uc@combtoksb
    \uc@prechar@exec{-1}%
    \global\uc@combtoksb{}%
      \ifx\uc@throw\undefined\else
        \def\uc@got{-1}\uc@throw\global\let\uc@throw\undefined\fi
  \else
    \noexpand\unicodecombine\fi
}
\uc@newcommand\uc@combine#1#2{%
  \ifx\protect\@typeset@protect
    \@temptokena\expandafter{#1{}}%
    \expandafter\expandafter\expandafter\ifx
    \expandafter\uc@firstofmany\the\@temptokena\uc@firstofmany\uc@cmb
      \uc@check@magicglue%
      \uc@combtoks\expandafter\expandafter\expandafter\expandafter
     \expandafter\expandafter\expandafter{%
        \expandafter\expandafter\expandafter\@gobble
        \expandafter#1\expandafter{\the\uc@combtoks}}%
    \else
      \unicode@combine%
      \xdef\uc@comb@code{\number#2}%
      \global\uc@combtoks\expandafter{#1{}}%
    \fi
    %\typeout{->COMBTOKS: \the\uc@combtoks}%
    \hskip\uc@magic@glue spplus0ptminus0pt %SPACE ; Insert magic glue
  \else
    \noexpand\unichar{\number#2}\fi
}
\uc@newcommand\uc@char@notloaded#1{%
  \count255=#1\divide\count255 by 256%
  \edef\uc@temp@a{uni-\number\count255.def}%
  \expandafter\ifx\csname\uc@temp@a\endcsname\relax\else
    \uc@secondtry#1\relax\fi
  \ifnum\uc@secondtry=#1\relax
    % If the file has already been loaded, but the character is unknown,
    % output an error and show the replacement glyph
    \unicode@numtohex\uc@temp@b{#1}4%
    \expandafter\ifx\csname
      missing-unicode-warned-\number#1\endcsname\relax
    \global\expandafter\let\csname
      missing-unicode-warned-\number#1\endcsname\@ne
      \unicode@error@unknown\@ne{Unknown Unicode character % SPACE
        \number#1 \uc@spc= U+\uc@temp@b,\MessageBreak
        possibly declared in \uc@temp@a.\MessageBreak
        Type H to see if it is available with options}{#1}%
    \else
      \PackageWarning{ucs}{Unknown character % SPACE
        \number#1 \uc@spc = 0x\uc@temp@b\uc@spc
        appeared again.}%
      \unicode@invalid{#1}%
    \fi
  \else
    \begingroup
    \ifUnicodeOptionsavemem
    \else
      \global\expandafter\let\csname\uc@temp@a\endcsname\@ne
    \fi
    \def\uc@got{#1}%
    \uni@resetcatcodes
    \expandafter\InputIfFileExists\expandafter{\uc@temp@a}{%
      \global\let\uni@dataloaded1%
      }{%
      }%
      % End of local group for inputted file
    \endgroup
      % Retry displaying character. This won't cause infinite recursion,
      % because we have marked this file as loaded (globally or, if
      % |savemem| is set, at least here).
    \uc@secondtry#1\relax%
    \uni@char{#1}%
  \fi
  }
\uc@newcommand\PreloadUnicodePage#1{%
  \begingroup
  \global\expandafter\let\csname uni-#1.def\endcsname\@ne
  \uni@resetcatcodes
  \InputIfFileExists{uni-#1.def}{\let\uni@dataloaded1}{%
    \PackageError{ucs}{Could not find uni-#1.def}{}}%
  \endgroup}
\uc@newcommand\PrerenderUnicode{%
  \@ifstar{\@prerenderunicode\unichar}{\@prerenderunicode\@gobble}}%
\uc@newcommand\@prerenderunicode#1#2{%
  \begingroup
  \UnicodeCharFilter\@gobble
  \let#1\@gobble\setbox0\hbox{#2}\endgroup}
\uc@newcommand\DeclareUnicodeCharacter#1#2{%
  \DeclareUnicodeCharacterAsOptional{#1}{document}{#2}}
\uc@newcommand\DeclareUnicodeCharacterAsOptional{%
  \let\uc@temp@a\relax\uni@declcharopt}
\uc@newcommand\uc@dclc#1#2{%
  \let\next=\uni@declcharopt
  \ifUnicodeOptionsavemem
    \ifnum\uc@got=#1\else
      \let\next=\@gobblethree\fi
  \fi
  \ifx\next\uni@declcharopt
    \expandafter\ifx\csname uni@active@#2\endcsname\relax
      \let\next\@gobblethree\else
    \expandafter\ifx\csname u-#2-\number#1\endcsname\relax\else
      \let\next\@gobblethree\fi\fi
    \let\uc@temp@a\global
  \fi
  \next{#1}{#2}}
\uc@newcommand\uni@declcharopt#1#2#3{%
  %\typeout{Defining: u-#2-\number#1 (\meaning\uc@temp@a)}%
  \ifx\utf@viii@map\undefined\else
    \expandafter\utf@viii@map\expandafter{\number#1}\fi
  \expandafter\uc@temp@a\expandafter\def
    \csname u-#2-\number#1\endcsname##1{#3}%\fi
  \expandafter\ifx\csname u-\number#1-h/o\endcsname\relax
    \expandafter\def\csname u-\number#1-h/o\endcsname{}\fi
  \expandafter\uc@temp@a\expandafter\edef
    \csname u-\number#1-h/o\endcsname{%
    {#2}\csname u-\number#1-h/o\endcsname}%
  }%
\let\unichar\uni@char
\uc@newcommand\unicodesuper#1{\textsuperscript{#1}}%
\uc@newcommand\@getcharinfo#1#2{%
  \begingroup
  \countdef\uc@got0\relax\uc@got#2\relax
  \global\def#1{Character's name unknown}%
  \def\info##1{\xdef#1{##1}}%
  \uni@resetcatcodes
  \ifUnicodeOptionfasterrors
  \global\def#1{No further informations known % SPACE
    because of option fasterrors.}\else
  {\InputIfFileExists{uninames.dat}{}{%
    \global\def#1{Character database uninames.dat not found. %SPACE
      \MessageBreak Character \number#2 \uc@spc unknown}}}%
  \fi
  \toks255{}%
  \def\uc@dclc##1##2##3{\ifnum##1=\uc@got
    \toks255\expandafter{\the\toks255, ##2}\fi}%
  \count255\uc@got\divide\count255by256\relax
  %\edef\temp@a{uni-\number\count255.def}%
  \InputIfFileExists{uni-\number\count255.def}{}{}%
  \expandafter\ifx\expandafter\@nil\the\toks255 \@nil
    \xdef#1{#1\noexpand\MessageBreak
      Character is not defined in uni-*.def files}%
  \else
    \expandafter\expandafter\expandafter\@getcharinfo@
    \expandafter\expandafter\expandafter#1%
    \expandafter\expandafter\expandafter
    {\expandafter#1\expandafter}\the\toks255 \@nil%
  \fi
  \endgroup}
\def\@getcharinfo@#1#2, #3\@nil{\gdef#1{#2\MessageBreak
    Character available with following options:\MessageBreak
    \uc@spc\uc@spc\uc@spc #3}}
\uc@newcommand\PrintUnicodeName#1{{%
  \@getcharinfo{\ci}{#1}%
  \def\MessageBreak{^^J}%
  \typeout{^^J\ci^^J}}}
\uc@newcommand\UnicodeCharFilter#1{\let\unicode@charfilter=#1}
\uc@newcommand\UCSProtectionNone{%
  \def\ucs@protected@unichar{}%
  \UnicodeCharFilter\@firstofone}
\uc@newcommand\UCSProtectionIeC{%
  \def\ucs@protected@unichar{}%
  \UnicodeCharFilter\IeC}
\uc@newcommand\UCSProtectionUnichar{%
  \def\ucs@protected@unichar##1{\ifx\protect\@typeset@protect}%
  \UnicodeCharFilter\@firstofone}
\UCSProtectionIeC
\uc@newcommand\uni@resetcatcodes{%
  \endlinechar=13\relax
  \def\reserved@a##1##2{%
    \@tempcnta##1\relax
    \@tempcntb##2\relax
    \reserved@b
    }%
  \def\reserved@b{%
    \ifnum\@tempcnta>\@tempcntb\else
    \reserved@c\@tempcnta
    \advance\@tempcnta\@ne
    \expandafter\reserved@b
    \fi
    }%
  \catcode`\ =10\relax
  \catcode`\#=6\relax
  \catcode`\$=3\relax
  \catcode`\%=14\relax
  \catcode`\&=4\relax
  \catcode`\\=0\relax
  \catcode`\^=7\relax
  \catcode`\_=8\relax
  \catcode`\{=1\relax
  \catcode`\}=2\relax
  \catcode`\~=13\relax
  \catcode`\@=11\relax
  \catcode`\^^I=10\relax
  \catcode`\^^J=12\relax
  \catcode`\^^L=12\relax
  \catcode`\^^M=5\relax
  \def\reserved@c##1{\catcode##1=12\relax}%
  \reserved@c{`\!}%
  \reserved@c{`\"}%
  \reserved@a{`\'}{`\?}%
  \reserved@c{`\[}%
  \reserved@c{`\]}%
  \reserved@c{`\`}%
  \reserved@c{`\|}%
  \def\reserved@c##1{\catcode##1=11\relax}%
  \reserved@a{`\A}{`\Z}%
  \reserved@a{`\a}{`\z}%
  \def\reserved@c##1{\catcode##1=15\relax}%
  \reserved@a{0}{`\^^H}%
  \reserved@c{`\^^K}%
  \reserved@a{`\^^N}{31}%
  \catcode"7F=15\relax
  \relax}
\catcode`\!13\relax
\uc@newcommand\unicode@error@unknown{\protect\unicode@error@unknown@}%
\uc@newcommand\unicode@error@unknown@#1#2#3{%
  {\expandafter\countdef\expandafter\uc@got\expandafter0%
     \expandafter\relax\expandafter\uc@got\number#3\relax
  \ifx\measuring@false\undefined\else\measuring@false\fi
  \@getcharinfo\uc@temp@c{#3}%
  \ifUnicodeOptionwarnunknown
    \PackageWarning{ucs}{#2\MessageBreak\uc@temp@c.\MessageBreak
        Enter I\noexpand!<RET> to define the glyph.}%
    \ifx#1\@ne\unicode@invalid{#3}\fi
  \else
    \let!\unicode@read@definition\catcode`\!13\relax
    \let\uc@read@definition\undefined
    \PackageError{ucs}{#2}{\uc@temp@c.\MessageBreak
        Enter I\noexpand!<RET> to define the glyph.}%
    \ifx#1\@ne
    \ifx\uc@read@definition\undefined\unicode@invalid{#3}%
    \else\uc@read@definition\fi\fi
  \fi}}
\catcode`\!12\relax
\uc@newcommand\unicode@read@definition{%
  \uni@resetcatcodes
  \typein[\definition]{Please enter definition for %SPACE
    unicode character \number\uc@got}%
  \global\let\uc@read@definition\definition
  \toks255\expandafter{\definition}%
  \edef\definition{\noexpand\DeclareUnicodeCharacter%
    {\number\uc@got}{\the\toks255}}%
  \toks255\expandafter{\definition}%
  \typeout{Tip:\MessageBreak You may include\MessageBreak
    \uc@spc\uc@spc\the\toks255\MessageBreak
    into your document source.}%
  \the\toks255\relax
  }
\def\uc@firstofmany#1#2\uc@firstofmany{#1}
\ifx\AtBeginDocument\undefined\else
\AtBeginDocument{\def\uc@tempa{\@inpenc@undefined@{utf8}}%
  \ifx\@inpenc@undefined\uc@tempa
  \ifx\restore@utf@viii@actives\undefined
  \PackageWarning{ucs}{***************************\MessageBreak You %SPACE
    seem to have loaded inputencoding utf8\MessageBreak (LaTeX kernel %SPACE
    UTF-8) instead of utf8x (ucs.sty UTF-8).\MessageBreak Probably you %SPACE
    are compiling a document written for a\MessageBreak
    pre-august-2004 ucs.sty.\MessageBreak
    ***************************\MessageBreak Please use %SPACE
    \string\usepackage[utf8x]{inputenc} instead of\MessageBreak
    \string\usepackage[utf8]{inputenc}.\MessageBreak
    ***************************\MessageBreak If you should really want %SPACE
    to use ucs.sty and kernel's\MessageBreak utf8.def together, use %SPACE
    \string\usepackage[utf8x,utf8]{inputenc}\MessageBreak to disable %SPACE
    compatibility mode\MessageBreak
    ***************************\MessageBreak Activating compatibility %SPACE
    mode.\MessageBreak ***************************\MessageBreak}%
  \global\let\uc@inputencoding\inputencoding
  \inputencoding{utf8x}%
  \def\inputencoding#1{%
    {\def\uc@tempa{#1}\def\uc@tempb{utf8}\ifx\uc@tempa\uc@tempb
      \aftergroup\@firstoftwo\else\aftergroup\@secondoftwo\fi}%
    {\restore@utf@viii@actives}{\uc@inputencoding{#1}}}%
  \fi\fi
}\fi

